Adaptive-saturated RNN: Remember more with less instability

Orthogonal parameterization is a compelling solution to the vanishing gradient problem (VGP) in recurrent neural networks (RNNs). With orthogonal parameters and non-saturated activation functions, gradients in such models are constrained to unit norms. On the other hand, although the traditional vanilla RNNs are seen to have higher memory capacity, they suffer from the VGP and perform badly in many applications. This work proposes Adaptive-Saturated RNNs (asRNN), a variant that dynamically adjusts its saturation level between the two mentioned approaches. Consequently, asRNN enjoys both the capacity of a vanilla RNN and the training stability of orthogonal RNNs. Our experiments show encouraging results of asRNN on challenging sequence learning benchmarks compared to several strong competitors. The research code is accessible at https://github.com/ndminhkhoi46/asRNN/.

==> Adaptive-saturated RNN_ Remember more with less instability/content/abstract.tex <==
%Recurrent Neural Networks (RNNs) has low trainability with long-term dependencies, which is often by caused the exploding and vanishing gradient problem (EVGP). In recent study, Tanh RNN is showed to have higher memory capacity than several other RNNs, despite being trade-off with an even lower trainability. Even though there are many techniques that relieve EVGP, few is known to work on Tanh RNN. In this article, we study the conditions for Tanh RNN to not vanish gradients. Such conditions allow a reconstruction of Tanh RNN, via linear transformation and initialization, into a variant called adapt-saturated RNN (asRNN). We compare asRNN against other models to show that asRNN maintains high memory capacity, trainability, and expressivity.

%Orthogonal parameterization has offered a compelling solution to the vanishing gradient problem (VGP) in recurrent neural networks (RNNs). Thanks to orthogonal parameters and non-saturated activation functions, gradients in such models are constrained to unit norms. On the other hand, although the traditional vanilla RNN have been observed to possess higher memory capacity, they suffer from the VGP and perform badly in many applications. This work connects the aforementioned approaches by proposing Adaptive-Saturated RNNs (asRNN), a variant that dynamically adjusts the saturation level between the two. Consequently, asRNN enjoys both the capacity of a vanilla RNN and the training stability of orthogonal RNNs. Our experiments show encouraging results of asRNN on challenging sequence learning benchmarks compared to several strong competitors. The research code is accessible at \href{https://github.com/ndminhkhoi46/asRNN/}{https://github.com/ndminhkhoi46/asRNN/}.

Orthogonal parameterization is a compelling solution to the vanishing gradient problem (VGP) in recurrent neural networks (RNNs). With orthogonal parameters and non-saturated activation functions, gradients in such models are constrained to unit norms. On the other hand, although the traditional vanilla RNNs are seen to have higher memory capacity, they suffer from the VGP and perform badly in many applications. This work proposes Adaptive-Saturated RNNs (asRNN), a variant that dynamically adjusts its saturation level between the two mentioned approaches. Consequently, asRNN enjoys both the capacity of a vanilla RNN and the training stability of orthogonal RNNs. Our experiments show encouraging results of asRNN on challenging sequence learning benchmarks compared to several strong competitors. The research code is accessible at \href{https://github.com/ndminhkhoi46/asRNN/}{https://github.com/ndminhkhoi46/asRNN/}.

==> Adaptive-saturated RNN_ Remember more with less instability/content/conclusion.tex <==
In the future, we plan to extend asRNN to scale-dependent loss (Assumption\ref{assumption:scaleindependent}). We also aim to reduce the computational cost using non-exponential sigmoids such as $\frac{x}{(1+|x|^k)^{k^{-1}}}$. %Ultimately, since memory capacity is observed to be a bottleneck in gated mechanisms \citep{collins2017capacity}, we hope to extend our work beyond vanilla RNN by investigating whether this problem is related to the VGP and whether we can do anything to change it.

As our work focuses on addressing the long memory and memory capacity problems of vanilla RNNs, we were unable to directly compare with relatively recent architecture such as UniCORNN for one key reason: they have multiple layers and more complex architectures such as stacked layers, gates, etc. In contrast, all methods we considered are related to the vanilla RNN with a single layer to demonstrate the main purpose of this study. In future works, we will consider improving asRNN for a fair comparison with more recent architectures.

==> Adaptive-saturated RNN_ Remember more with less instability/content/experiment.tex <==
\begin{figure}[t]
	\subfloat[Copy task ($L=2000$) \label{copy2000fig}]	{\includegraphics[width=5.4cm]{./content/copy_2000.png}}
	\subfloat[Sequential MNIST\label{smnistfig}]{\includegraphics[width=4.293cm]{./content/sMNIST.png}}
	\subfloat[Permuted MNIST\label{pmnistfig}]{\includegraphics[width=4.293cm]{./content/pMNIST.png}}
	\caption{Training loss for the Copy task and test accuracies for the sequential and permuted MNIST.\label{fig}}
	\vspace*{-0.2in}
\end{figure}
\begin{wraptable}{r}{0.42\textwidth}
	\small
	\begin{center}
		\setlength\tabcolsep{3pt}
		\begin{tabular}{|l|c|c|}
			\hline
			Model & $T=150$ & $T=300$  \\ \hline
			LSTM & $\bm{1.41 \pm 0.005}$ & $\bm{1.43 \pm 0.004}$  \\ \hline
			asRNN & $1.46 \pm 0.006$ & $1.49 \pm 0.005$  \\ \hline
			nnRNN & $1.47 \pm 0.003$ & $1.49 \pm 0.002$  \\ \hline
			expRNN & $1.49 \pm 0.008$ & $1.52 \pm 0.001$  \\ \hline
			EURNN & $1.61 \pm 0.001$ & $1.62 \pm 0.001$ \\ \hline
			RNN-orth & $1.62 \pm 0.004$ & $1.66 \pm 0.006$  \\ \hline
			RNN & $2.89 \pm 0.002$ & $2.90 \pm 0.002$  \\ \hline
		\end{tabular}
		\captionof{table}{Test BPC on PTB-c at different BPTT lengths (T). Best results are in bold.}\label{ptbctab}
		\vspace*{-0.2in}
	\end{center}
\end{wraptable}

To validate the model's memory capacity, we consider the Copy task\citep{10.1162/neco.1997.9.8.1735}, sequential MNIST\citep{lecun1998gradient}, and permuted MNIST\citep{GoodfellowMDCB13}. Next, we use the Penn Treebank character-level prediction (PTB-c)\citep{marcus-etal-1993-building} task to explore the model's expressivity \citep{10.5555/3454287.3455506, Bojanowski2015AlternativeSF}. We benchmark asRNN against the strong orthogonal RNNs with long memories and high trainability such as expRNN\citep{pmlr-v97-lezcano-casado19a}, scoRNN\citep{pmlr-v80-helfrich18a}, uRNN\citep{pmlr-v48-arjovsky16}, and the popular LSTM\citep{10.1162/neco.1997.9.8.1735} with high expressivity from the gated mechanism. We follow the setting described in Appendix~\ref{experiment} and report the results in Fig.~\ref{fig} and Tab.~\ref{ptbctab}. On long sequence learning tasks (Fig.~\ref{fig}), our asRNN shows excellent performance by converging stably on the Copy task, and achieves better generalization on the sequential and permuted MNIST tasks. On the PTB task, asRNN achieved encouraging results by outperforming all orthogonal RNN baselines, only second to LSTM. Overall, our empirical results show that asRNN possesses both high memory capacity and expressivity compared to other non-gated RNNs and can alleviate the EVGP, which corroborates our motivation in Sec.~\ref{sec:introduction}.

\vspace*{-0.05in}
\section{Conclusion}
\vspace*{-0.05in}
We have investigated the potential and limitations of vanilla RNNs in learning long-sequence tasks. Then, we proposed asRNN, a novel vanilla RNN variant that enjoys strong resistance to the VGP and can possess long memory. Our experiment results show asRNN enjoys encouraging performances on tasks that demand memory span, memory capacity, or expressivity.
%In this work, we propose asRNN, a novel variant of vanilla RNN. Under mild assumptions and conditions, we show that asRNN does not exhibit the VGP and potentially possesses long memory. We also conduct experiments to demonstrate asRNN superior trainability on tasks requiring high memory capacity and expressivity.
%Under mild conditions, the proposed asRNN successfully mitigates VGP to possess long memory through orthogonal RNN mechanisms. We provided theoretical arguments and experiments to justify asRNN's superior ability on tasks demanding memory span, memory capacity, and expressivity.
\if0
We compare memory capacity of each model using copy memory task (recall length of $10$, delay length of $2000$) and pixelated MNIST tasks. We also use Penn Tree Bank character-level prediction (PTB-c) task, which do not bottleneck memory capacity, to compare the models \citet{collins2017capacity}. A key factor deciding good performance on such task is the expressiveness, including structural design and the hidden size \citep{Bojanowski2015AlternativeSF}. We benchmark asRNN against several unitary-based RNNs, which has high memory capacity \citep{10.5555/3045390.3045605}, and with LSTM, which has high expressiveness. Appendix~\ref{experiment} provides details of the data sets and the experimental setup.

Figure~\ref{copy2000fig}, Figure~\ref{smnistfig}, and Figure~\ref{pmnistfig} show that asRNN outperforms unitary-based RNNs and LSTM at both memorization and trainability. Good convergence on such tasks indicates asRNN successes at learning long-term dependencies without vanishing gradient. In Table~\ref{ptbctab}, asRNN performs only second to the gated mechanism LSTM. The result shows that asRNN possesses high memory capacity, trainability, and expressiveness on hidden state.
\begin{figure}[thbp]
	\subfloat[Train losses at copy memory (L=2000).\label{copy2000fig}]	{\includegraphics[width=4.94cm]{./content/copy_2000.png}}
	\subfloat[Best test accuracy at sMNIST.\label{smnistfig}]{\includegraphics[width=4.4cm]{./content/sMNIST.png}}
	\subfloat[Best test accuracy at pMNIST.\label{pmnistfig}]{\includegraphics[width=4.4cm]{./content/pMNIST.png}}
	\caption{Memorization benchmarks.}
\end{figure}
\begin{wrapfigure}[10]{r}{0.5\textwidth}
	\begin{center}
		\begin{tabular}{|l|l|l|}
			\hline
			Model & T=150 & T=300  \\ \hline
			LSTM & {\bf 1.41 ± 0.005} & {\bf 1.43 ± 0.004}  \\ \hline
			asRNN & 1.46 ± 0.006 & 1.49 ± 0.005  \\ \hline
			nnRNN* & 1.47 ± 0.003 & 1.49 ± 0.002  \\ \hline
			expRNN* & 1.49 ± 0.008 & 1.52 ± 0.001  \\ \hline
			EURNN* & 1.61 ± 0.001 & 1.62 ± 0.001 \\ \hline
			RNN-orth* & 1.62 ± 0.004 & 1.66 ± 0.006  \\ \hline
			RNN* & 2.89 ± 0.002 & 2.90 ± 0.002  \\ \hline
		\end{tabular}
		\captionof{table}{Test bit-per-character at PTB-c.}\label{ptbctab}
	\end{center}
\end{wrapfigure}
\fi

==> Adaptive-saturated RNN_ Remember more with less instability/content/methodology.tex <==
\textbf{Formulation } Based on the observation Eq.~\ref{eqn:motivation}, we formally define the hidden cell of asRNN as:
\begin{equation}
	h_t = \mW_f^{-1}\mathrm{tanh}( \mW_f( \mW_{xh}\vx_{t}+ \mW_{hh}\vh_{t-1} + \vb)),
\end{equation}
where $\gW=\{\mW_f, \mW_{xh}$, $\mW_{hh}, \vb\}$ is the set of trainable parameters, $\mW_f$ introduces an end-to-end composite layer to control the saturation level of asRNN. To ensure the non-singularity of $\mW_f$, we parameterize $\mW_f = \mU_f \mD_f$, where $\mU_f$ is orthogonal, $\mD_f$ is positively diagonal. Remarkably, we observe that: (i) by fixing  $\mW_f$ to be identity, we recover a vanilla RNN; and (ii) let $\mW_{hh}$ be orthogonal, fix $\mU_f$ to be the identity, and let $\mD_f \to \mathbb{0}$, we recover an orthogonal RNN. From such construction, asRNN not only dynamically adjusts the saturation level but also controls the singular values of the temporal Jacobian (Thm.~\ref{maintheoremlabel}), which in turn alleviates the VGP.

\textbf{Key theoretical result }
Let $\vw \in \gW$, we define the gradient and Jacobian as~\citep{Pascanu2012OnTD}: $\frac{\partial \Lagr}{\partial \vw} = \sum_{1 \leq t_1 \leq T}\frac{\partial \Lagr}{\partial \vh_T}\mJ( T,t_1) \frac{\partial \vh_{t_1}}{\partial \vw}$, where
$\mJ( t_2,t_1)  =  \prod_{t_1 < t \leq t_2} \mJ( t) $ and $\mJ(t) = \mW_f^{-1}\text{diag}[1-( \mW_f\vh_t) ^2]\mW_f\mW_{hh}$.
The vanishing gradient problem in RNNs is credited to the existence of a temporal Jacobian $\mJ(t_2,t_1) \approx 0$ that bottlenecks the backpropagated signal. 
Under mild assumptions (Appendix~\ref{appendix:assumption}), we show a condition for asRNN where all singular values of temporal Jacobian matrices are lower bounded by $1$. Thanks to this, the VGP is alleviated on vanilla RNN.
\begin{restatable}{theorem}{maintheoremrestate}\label{maintheoremlabel}
	Let $G$ and $H$ be respectively the $d_h$-th degree generalized permutation group and its signed permutation subgroup. Under the assumptions in Appendix~\ref{appendix:assumption}, if $\norm{\mD_{f}}_2\leq \frac{\text{arctanh}( \sqrt{1-\norm{\mW_{hh}^{-1}}_2}) }{(\norm{\mW_{xh}}_2C_x + \norm{\vb}_\infty) \sum_{i=0}^{t-1}( \norm{\mW_{hh}}_{\max}+1)^i}$ and
	$\min_{\mE\in G}\norm{\mW_{hh} - \mE}_2 \leq \frac{\sigma_{\min}( \mD_{f})}{\norm{\mD_{f}}_2}$, then
	$$\forall t_2>t_1\in\mathbb{N}^*, \exists \epsilon\geq0: \min_{\mE\in H}\norm{\mU_{f} - \mE}_2 \leq \epsilon  \rightarrow  \sigma_{\min}(\mJ(t_2,t_1))\geq 1.$$
\end{restatable}
\vspace*{-0.1in}
Importantly, while \citet{pmlr-v119-zhao20c} questioned and showed a scenario where vanilla RNN and LSTM have a short memory, a problem associated with the VGP. In contrast, our Thm.~\ref{maintheoremlabel} suggests the existence of another in which vanilla RNN resists VGP and possesses long memory.%\citet{pmlr-v119-zhao20c} conjectured and showed a scenario where RNNs and LSTM have short-term memories, a problem associated with the VGP. Thm.~\ref{maintheoremlabel} shows another where vanilla RNN does not exhibit the VGP. Hence, the conjecture of \citet{pmlr-v119-zhao20c} is suggested to be false.

%Importantly, \citet{pmlr-v119-zhao20c} conjectured and showed a case where RNN and LSTM have short memories, a problem associated with the VGP, from a statistical perspective. Here, we show another case where a vanilla RNN variant does not exhibit the VGP. Our result suggests the conjecture of \citet{pmlr-v119-zhao20c} might not hold true in general.

\if0
Across this article, $d_h, T \in \mathbb{N}$ denote respectively the hidden size and the sequence length. The symbols $\Lagr$ and $\theta$ stand respectively for a scale-independent loss (Assumption~\ref{scaleindependent}) and a scalar parameter of asRNN. For simple notation, the proof assumes many-to-one tasks. However, the result also generalizes to other tasks.

Generalized from the observation in section~\ref{sec:introduction}, we reconstructs Tanh RNN as following: $ \mW_f^{-1}\text{tanh}( \mW_f( \mW_{xh}\vx_{t}+ \mW_{hh}\vh_{t-1} + \vb) ) $, where $\mU_f$ is orthogonal, $\mD_f$ is positive diagonal and $\mW_f=\mU_f\mD_f$. Similar to \citet{Pascanu2012OnTD}, $\frac{\partial \Lagr}{\partial \theta} = \sum_{1 \leq t_1 \leq T}\frac{\partial \Lagr}{\partial \vh_T}\mJ( T,t_1) \frac{\partial \vh_{t_1}}{\partial \theta}$, where
$\mJ( t_2,t_1)  =  \prod_{t_1 < t \leq t_2} \mJ( t) $ and $\mJ(t) = \mW_f^{-1}\text{diag}[1-( \mW_f\vh_t) ^2]\mW_f\mW_{hh}$.

The vanishing gradient problem in RNNs can be credited to the existence of a temporal Jacobian $\mJ(t_2,t_1) \approx 0$ that bottlenecks the back-propagated signal. The next theorem states that under assumptions in Appendix~\ref{assumptionappendix}, there is a configuration of asRNN such that every singular value of the temporal Jacobian matrix is lower bounded by $1$. In other words, there is no vanishing gradient.
\begin{restatable}{theorem}{maintheoremrestate}\label{maintheoremlabel}
  Let $G$ and $H$ be respectively the $d_h$-th degree generalized permutation group and its signed permutation subgroup. Under the assumptions in Appendix~\ref{assumptionappendix}, if $\norm{\mD_{f}}_2\leq \frac{\text{arctanh}( \sqrt{1-\norm{\mW_{hh}^{-1}}_2}) }{(\norm{\mW_{xh}}_2C_x + \norm{\vb}_\infty) \sum_{i=0}^{t-1}( \norm{\mW_{hh}}_{\max}+1)^i}$ and
  $\min_{\mE\in G}\norm{\mW_{hh} - \mE}_2 \leq \frac{\sigma_{\min}( \mD_{f})}{\norm{\mD_{f}}_2}$, then
  $$\exists \epsilon\geq0: \min_{\mE\in H}\norm{\mU_{f} - \mE}_2 \leq \epsilon  \rightarrow \forall t_2>t_1\in\mathbb{N}^*: \sigma_{\min}(\mJ(t_2,t_1))\geq 1.$$
\end{restatable}
Details on how the configuration integrates into asRNN is detailed in Appendix~\ref{subsec:expsetup}.
\fi


==> Adaptive-saturated RNN_ Remember more with less instability/content/motivation.tex <==
\label{sec:introduction}
Training vanilla RNNs (with tanh activation) is notoriously challenging due to the VGP, where the gradients' magnitudes become \emph{exponentially} smaller~\citep{collins2017capacity}. Thus, extensive efforts have been devoted to develop more stable, effective models such as orthogonal RNNs~\citep{pmlr-v97-lezcano-casado19a}, and LSTM~\citep{10.1162/neco.1997.9.8.1735}. Empirically, orthogonal RNNs show more competitive performances compared to LSTM and vanilla RNN on long-sequence tasks. However, due to non-saturated activations and unitary constrain, their memory capacity is also more limited compared to vanilla RNN~\citep{collins2017capacity}. 

This study aims to realize the memory capacity potential of vanilla RNNs by endowing them with the capability to address the VGP of orthogonal RNNs. As a result, we propose the \emph{adaptive-saturated RNN} (asRNN), a vanilla RNN variant that dynamically adjusts the activation's saturation level. Particularly, we observe that, let $f(x;a) = \frac{\mathrm{tanh} (ax)}{a}$, then:
\begin{equation} \label{eqn:motivation}
\lim_{a \to 0} f(x;a)=x, \quad \mathrm{and} \quad \lim_{a \to 1} f(x;a) = \mathrm{tanh}(x).
\end{equation}
Thus, by generalizing and using $f(x;a)$ as an activation function, we can adjust $a$ and update the parameters freely of a vanilla RNN to achieve high memory capacity without being affected by the VGP. In the following, we will formally introduce asRNN and outline a key result of a condition for avoiding the VGP in asRNN. 

%By adjusting $a$ and updating parameters with more freedom than an orthogonal RNN, it is possible to have high memory capacity without being affected by the VGP, thereby maintaining high training stability. Moreover, by generalizing and using $f(x;a)$ as an activation function, we also control gradient norms. 
%Remarkably, adjusting $a$ mitigates the exploding gradient problem (EGP), which is achievable with gradient clipping (Appendix~\ref{common_setting}). Next, we formally introduce asRNN and outline a key result of a condition for avoiding the VGP in asRNN. Finally, we demonstrate asRNN's promising performance on challenging sequence learning problems against several strong competitors.

\if0
In \citet{Pascanu2012OnTD}, RNN is shown to have low trainability, displayed with unstable convergence, or converging to bad optimums when learning long-term dependencies. The same source associated this low trainability with the vanishing and exploding gradient problems (EVGP), the exponential changes in the scale of gradients induced by the re-application of hidden parameters. Observed in \citet{collins2017capacity}, Tanh RNN has lower trainability but also stores more task information per parameter than ReLU RNN, GRU, and LSTM.  In \cite{pmlr-v119-zhao20c}, the authors proved that over an infinite time scale and under scale-dependent loss (MSE in the original article; see Assumption~\ref{scaleindependent}), Tanh RNN does not possess long-term memory and might exhibit vanishing gradient problem.

In this article, by observing $ f(a,x)=a\text{tanh}(\frac{x}{a})$ is a $1$-Lipschitz function satisfying $\lim_{a\to 0}f(a,x)=x$, we notice that Linear RNN solutions can also be approximated by a Tanh RNN. Leveraging this observation, we prove the existence of conditions under which Tanh RNN does not vanish gradient. The conditions allow us to reparameterize and initialize Tanh RNN into a variant called adapt-saturated RNN (asRNN).

We compare asRNN with LSTM and unitary-based RNNs at long sequential classification to show that without vanishing gradient, our variant possesses high memory capacity and trainability. Furthermore, since singular values and eigenvalues of $\mJ(t)$ (see section~\ref{sec:method}) in asRNN is less restricted than unitary-based RNNs, we speculate our model to perform better on tasks requiring large hidden size or complex structural design such as language modeling. This speculation will be put to test.
\fi

==> Adaptive-saturated RNN_ Remember more with less instability/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

